Continual Learning for Segment Anything Model Adaptation

Although the current different types of SAM adaptation methods have achieved promising performance for various downstream tasks, such as prompt-based ones and adapter-based ones, most of them belong to the one-step adaptation paradigm. In real-world scenarios, we are generally confronted with the dynamic scenario where the data comes in a streaming manner. Driven by the practical need, in this paper, we first propose a novel Continual SAM adaptation (CoSAM) benchmark with 8 different task domains and carefully analyze the limitations of the existing SAM one-step adaptation methods in the continual segmentation scenario. Then we propose a novel simple-yet-effective Mixture of Domain Adapters (MoDA) algorithm which utilizes the Global Feature Tokens (GFT) and Global Assistant Tokens (GAT) modules to help the SAM encoder extract well-separated features for different task domains, and then provide the accurate task-specific information for continual learning. Extensive experiments demonstrate that our proposed MoDA obviously surpasses the existing classic continual learning methods, as well as prompt-based and adapter-based approaches for continual segmentation. Moreover, after sequential learning on the CoSAM benchmark with diverse data distributions, our MoDA maintains highly competitive results in the natural image domain, approaching the zero-shot performance of the original SAM, demonstrating its superior capability in knowledge preservation. Notably, the proposed MoDA can be seamlessly integrated into various one-step adaptation methods of SAM, which can consistently bring obvious performance gains. Code is available at \url{https://github.com/yangjl1215/CoSAM}

==> sec/intro_ori.tex <==


\section{Introduction}
\yi{Image segmentation is a foundational task in computer vision~[CITE XXX], essential for enabling machines to understand and interpret visual content across a wide range of applications. Recently, the method Segment Anything Model (SAM)~\cite{sam} has introduced a groundbreaking shift in this field, achieving an unprecedented level of versatility and accuracy. With its ability to perform high-quality segmentation across diverse settings, SAM represents a major leap forward, setting new benchmarks and significantly expanding the scope of automated segmentation.}

% The Segment Anything Model (SAM) \cite{sam} marks substantial progress in computer vision, demonstrating notable versatility and accuracy in image segmentation. However, recent research indicates that SAM does not always maintain satisfactory performance, particularly in certain sub-domains \cite{sam_struggle_chengmingming, sam_not_perfect, sam_adapter}, falling short of its bold claim to \emph{segment anything}.

% To overcome SAM's limitations, researchers have developed various strategies to boost its performance across new domains. For instance, SAM-Adapter \cite{sam_adapter} integrates multiple learnable MLP Blocks to enhance segmentation in complex scenarios like camouflage detection and polyp segmentation. Surgical-SAM \cite{surgical_sam} uses Low Rank Adaptation (LoRA) \cite{lora} for increased accuracy in robotic surgery. Additionally, techniques such as HQ-SAM \cite{sam_hq} and MSA \cite{msa} employ adapters with diverse structures to tailor SAM for various granularities and modalities, demonstrating proactive efforts to improve its efficacy in specific domains.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{./figures/all_radar_charts.png}
	\caption{Performance comparison of each SAM adaptation method on our Co-SAM Benchmark. \textcolor[HTML]{48AFC7}{Blue} indicates the IoU for each task when the model is just fine-tuned on that specific task, while \textcolor[HTML]{D43434}{red} shows the IoU after sequential training across all tasks. The sequential training process begins with BSData (moving clockwise) and concludes with Polyp.}
    \label{radar_chart}
\end{figure}
\yi{Although SAM provides a solid foundation for segmentation tasks, recent studies indicate that its performance is limited in certain specific sub-domains~\cite{sam_struggle_chengmingming, sam_not_perfect, sam_adapter}. To address this issue, various algorithms have been developed, each proposing different strategies to enhance SAM’s performance on downstream tasks. For instance, SAM-Adapter~\cite{sam_adapter} integrates multiple learnable MLP Blocks to enhance segmentation in complex scenarios like camouflage detection and polyp segmentation. Surgical-SAM \cite{surgical_sam} uses Low-Rank Adaptation (LoRA) \cite{lora} for increased accuracy in robotic surgery. Moreover, techniques such as HQ-SAM \cite{sam_hq} and MSA \cite{msa} employ adapters with diverse structures to tailor SAM for various granularities and modalities, demonstrating proactive efforts to improve its efficacy in specific domains.} 

\yi{However, these methods primarily rely on one-step adaptation, which is limited in real-world scenarios where models face continuous data streams and need ongoing updates. In such dynamic scenarios, one-step adaptation methods focus solely on the most recently finetuned task, making it difficult for models to handle new tasks while preserving performance on previous ones. 
% one-step adaptation methods make it difficult for the model to adapt to new tasks while maintaining performance on previous tasks.
% In such dynamic scenarios, one-step adaptation struggles to capture the evolving patterns needed to sustain high performance and avoid severe forgetting. 
Therefore, how to utilize the capabilities of SAM across a sequence of continual tasks to quickly adapt to new tasks while maintaining the performance of old tasks is a challenging problem. To investigate SAM's potential in the continual scenario, we construct a benchmark for continual segmentation, called Continual SAM Adaptation Benchmark (Co-SAM), which aims to systematically evaluate SAM-related algorithms's performance within the streaming scenarios. Specifically, Co-SAM offers a set of eight tasks covering diverse domains, including industrial defects, medical imaging, and camouflaged objects, to serve as a realistic and effective benchmark for evaluating current methods.       }  

\yi{Leveraging the constructed Co-SAM, we select six representative continual learning (CL) algorithms, modify and integrate them into SAM, and evaluate their performance.  Specifically, these CL algorithms include classic methods such as LWF \textbf{[CITE]}, EWC, and ER, along with recent, more competitive prompt-based methods like L2P, Dual-Prompt, and Conda-Prompt. These prompt-based methods typically construct a prompt pool containing key-value pairs of tokens. By matching the image features extracted by pre-trained model with the well-learned key tokens, the model can utilize the corresponding value tokens as the task-specific information to boost performance. However, the results indicate that although these CL algorithms perform well on classification tasks with foundation models, their performance on continual segmentation tasks is less satisfactory. This highlights the urgent need to address the continual segmentation problem with foundation models. }

\yi{By analyzing the reasons behind the suboptimal performance of leading prompt-based CL classification methods on our proposed continual segmentation benchmark, Co-SAM, we identified two key factors: 1) The key tokens learned by classification-based CL methods differ from those learned through the SAM encoder, which is specifically designed to interact with user inputs and prioritize local information over global features. Thus, their designed key tokens are not well-suited for differentiating for SAM-based CL algorithms.~2) Even when key token matching is accurate, incorporating value tokens alone does not lead to significant performance improvements in segmentation tasks. [\textbf{REWRITE}]}

\yi{To address these issues, we propose the Mixture of Domain Adapters (MoDA) algorithm. Firstly, we introduce the Global Feature Tokens (GFT) and Global Assistant Tokens (GAT) modules, which enable the pre-trained segmentation encoder to capture global features for improved differentiation. By interacting with image tokens at each layer of the transformer within the frozen SAM network, the model can extract task-specific information that represents the global features of the input image. Secondly, we replace the value tokens with adapters better suited to modulate the spatial and channel-wise structure of the feature maps. \textbf{xxxxx}} To sum up,  our contributions can be summarized as follows:
 \begin{itemize}[leftmargin=3.5mm, itemsep=0mm, topsep=-0.5 mm]
    \item[$\circ$] \yi{We establish the novel Co-SAM benchmark to assess the performance of SAM-based CL algorithms, providing a key platform for future research on the effectiveness of Continual Learning methods with segmentation-based foundational models.}
    % We establish the novel Co-SAM Benchmark to assess the performance of SAM adaptation algorithms in a Continual Learning context, serving as a crucial platform for future research to test Continual Learning methods' applicability in the context of foundational model adaptation.
    \item[$\circ$] \yi{We implement and analyze why current top-performing CL methods struggle on Co-SAM. Building on these insights, we propose the MoDA algorithm, which integrates the GFT and GAT modules, along with XXX.}
    \item[$\circ$] \yi{We conduct comprehensive experiments and ablation studies to demonstrate the effectiveness of the proposed MoDA algorithm.}
    % Third, we develop Mixture of Domain Adapters (MoDA), a simple yet highly effective task-adaptive approach that makes SAM more versatile as a foundational model in computer vision, and able to evolve in a dynamic and diverse environment.
\end{itemize}

% the key tokens learned in classification-based CL methods are not suitable for segmentation tasks because SAM encoder is specifically designed to interact with user inputs, emphasizing local information over global distinctions, thus the key matching part is not accurate; 2) even when key token matching is correct, simply adding value tokens does not yield satisfactory performance improvements. }

% they focus on global features, whereas segmentation requires emphasis on localized information.}
% Despite their excellent performance, these methods are confined to the mindset of \emph{one-step adaptation}—collecting data from underperforming domains and then fine-tuning SAM on this data, often resulting in a model optimized for just one specific dataset.

%Pursuing the goal of ``segment anything" with a one-step adaptation mindset assumes the impractical task of exhaustively collecting data from all underperforming domains—a fundamentally flawed premise. New domains constantly emerge, requiring ongoing adaptation. 

Current one-step adaptation methods are limited in their ability to accommodate continually changing domains. For instance, a household robot will encounter a constantly evolving set of household objects, requiring it to continuously learn to understand new items. This necessitates the introduction of Continual Learning (CL) into SAM Adaptation.

Furthermore, numerous Continual Learning algorithms have been proposed for classification tasks. We tested both traditional CL methods and the more recent prompt-based CL algorithms, which leverage pre-trained models, on the task of SAM Continual Adaptation. The performance of these methods on Co-SAM falls short of their effectiveness in classification tasks, suggesting that approaches developed for classification cannot be directly applied to SAM Continual Adaptation.


\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{./figures/Co-SAM_pipeline2.png}
	\caption{The workflow of the Co-SAM Benchmark. Each method undergoes training on a sequence of tasks and is evaluated on all seen tasks along the course.}
        \label{Co-SAM_pipeline}
\end{figure}

For these reasons, we introduce the Continual SAM Adaptation Benchmark (Co-SAM), specifically designed to evaluate the performance of various SAM adaptation algorithms within a Continual Learning framework. Co-SAM also helps to highlight the limitations of existing CL methods originally developed for classification, facilitating the development of improved algorithms. Co-SAM includes a suite of eight tasks spanning a variety of domains such as industrial defects, medical imaging, and camouflaged objects, ensuring a comprehensive evaluation across diverse settings.

%Given that no existing methods suitably evaluate our Co-SAM Benchmark, we reproduced six Continual Learning methods. While these methods mitigate forgetting to some extent, they do not fully meet our needs. 


We reproduced six existing CL methods originally developed for classification tasks and observed that the more recent prompt-based methods (L2P, Dual-Prompt, Coda-Prompt) performed even worse than the traditional methods (LwF, EWC, ER). This is unexpected, as prompt-based methods are designed to leverage large pre-trained models, which should theoretically enhance compatibility in SAM adaptation. Specifically, these prompt-based methods build a prompt pool containing key-value pairs of tokens. Image features extracted by the pre-trained model are used to match with key tokens in the prompt pool, and the corresponding value tokens are concatenated with image patch tokens before being fed into the model. During training, key tokens are adjusted to align more closely with the image features, while value tokens are trained to provide task-specific context, helping the pre-trained model adapt to different tasks. The poor performance of prompt-based methods on the Co-SAM Benchmark appears to stem from \textit{two main issues}. \textit{First}, key token matching is frequently inaccurate. When value tokens optimized for one task are matched with another task, significant performance degradation occurs. \textit{Second}, even when key token matching is correct, simply adding value tokens does not yield satisfactory performance improvements.

To address these issues, we propose Mixture of Domain Adapters (MoDA).

\textit{First}, we identified that the challenge with ineffective matching in segmentation tasks, despite successful matching in classification tasks, arises from differences in the characteristics of the features extracted by the pre-trained model.

In classification tasks, prompt-based methods effectively utilize the ImageNet-pre-trained encoder’s capacity for extracting high-level global features, resulting in well-separated key tokens across different tasks. However, the SAM encoder is specifically designed to interact with user inputs, such as points or bounding boxes, to produce localized masks, emphasizing local information over global distinctions. As a result, key tokens in this setting are not well-suited for differentiating between tasks.

To enable the pre-trained segmentation encoder, originally focused on extracting local features, to also capture global features, we introduce Global Feature Tokens (GFT) and Global Assistant Tokens (GAT) in MoDA. These tokens interact with image tokens at each layer of the transformer within the frozen SAM network, allowing the model to extract task-specific information that represents the global features of the input image. This, in turn, enables more precise querying and provides task-specific guidance, facilitating better segmentation performance.

\textit{Second}, we replace the value tokens with adapters better suited to modulate the spatial and channel-wise structure of the feature maps. The concatenated value tokens are sufficient to modulate the high-level feature space and influence the classification decision. However, segmentation requires precise, spatially detailed feature transformations to accurately delineate object boundaries and regions, so as to enable the model to produce accurate pixel-wise predictions.


To sum up,  our contributions can be summarized as follows:
 \begin{itemize}[leftmargin=3.5mm, itemsep=0mm, topsep=-0.5 mm]
    \item[$\circ$] First, we establish the novel Co-SAM Benchmark to assess the performance of SAM adaptation algorithms in a Continual Learning context, serving as a crucial platform for future research to test Continual Learning methods' applicability in the context of foundational model adaptation.
    \item[$\circ$] Second, we reproduce a set of Continual Learning strategies on the Co-SAM Benchmark. The insights gained from these implementations encourage exploration into effective continual learning strategies.
    \item[$\circ$]  Third, we develop Mixture of Domain Adapters (MoDA), a simple yet highly effective task-adaptive approach that makes SAM more versatile as a foundational model in computer vision, and able to evolve in a dynamic and diverse environment.
    
    
 \end{itemize}

% \section{Introduction}
% \label{sec:intro}

% Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
% This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

% %-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}

